Isotropy and Log-Concave Polynomials: Accelerated Sampling and High-Precision Counting of Matroid Bases

We define a notion of isotropy for discrete set distributions. If $\mu$ is a distribution over subsets $S$ of a ground set $[n]$, we say that $\mu$ is in isotropic position if $P[e \in S]$ is the same for all $e\in [n]$. We design a new approximate sampling algorithm that leverages isotropy for the class of distributions $\mu$ that have a log-concave generating polynomial; this class includes determinantal point processes, strongly Rayleigh distributions, and uniform distributions over matroid bases. We show that when $\mu$ is in approximately isotropic position, the running time of our algorithm depends polynomially on the size of the set $S$, and only logarithmically on $n$. When $n$ is much larger than the size of $S$, this is significantly faster than prior algorithms, and can even be sublinear in $n$. We then show how to transform a non-isotropic $\mu$ into an equivalent approximately isotropic form with a polynomial-time preprocessing step, accelerating subsequent sampling times. The main new ingredient enabling our algorithms is a class of negative dependence inequalities that may be of independent interest. As an application of our results, we show how to approximately count bases of a matroid of rank $k$ over a ground set of $n$ elements to within a factor of $1+\epsilon$ in time $ O((n+1/\epsilon^2)\cdot poly(k, \log n))$. This is the first algorithm that runs in nearly linear time for fixed rank $k$, and achieves an inverse polynomially low approximation error.

==> style.tex <==
\makeatletter


% -- Options

\RequirePackage{options}

\options{
	/opts/.new family,
	/opts/colors/.new toggle=true,
	/opts/fonts/.new toggle=true,
	/opts/math/.new toggle=true,
	/opts/theorems/.new toggle=true,
	/opts/macros/.new toggle=true,
	/opts/graphics/.new toggle=true,
	/opts/tools/.new toggle=true,
	/opts/typesetting/.new toggle=true,
	/opts/biblio/.new toggle=true
}
\options{/opts}

\providetoggle{presentation}
\@ifclassloaded{beamer}{\toggletrue{presentation}}{\togglefalse{presentation}}

% -- Packages

\iftoggle{/opts/math}{
	\RequirePackage{amsmath}
	\RequirePackage{amssymb}
	\RequirePackage{bm}
	\RequirePackage{dsfont}
	\RequirePackage{mathtools}
}{}

\iftoggle{/opts/theorems}{
	\RequirePackage{amsthm}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikz}
	\RequirePackage{tikz-3dplot}
	\RequirePackage{tcolorbox}
	\RequirePackage{pgfplots}
	\RequirePackage{tcolorbox}
	\pgfplotsset{compat=newest}
}{}

\iftoggle{/opts/tools}{
	\RequirePackage[ruled]{algorithm2e}
	\RequirePackage{datatool}
	\RequirePackage[super]{nth}
	\RequirePackage{scalerel}
	\iftoggle{presentation}{}{
		\RequirePackage[shortlabels]{enumitem}
	}
}{}

\iftoggle{/opts/fonts}{
	\iftoggle{presentation}{}{
		\RequirePackage[sc]{mathpazo}
	}
}{}

\iftoggle{/opts/biblio}{
	\iftoggle{presentation}{}{
		\RequirePackage[backend=biber, style=alphabetic, maxbibnames=99, maxcitenames=99, url=false]{biblatex}
	}
}

\iftoggle{/opts/colors}{
	\newcommand{\declarecolor}[2]{\@ifundefined{\string\color@#1}{\definecolor{#1}{RGB}{#2}\expandafter\newcommand\csname #1\endcsname[1]{\textcolor{#1}{##1}}}{}}
	\declarecolor{Black}{0, 0, 0}
	\declarecolor{White}{255, 255, 255}
	\declarecolor{Gray}{127, 127, 127}
	\declarecolor{LightGray}{216, 216, 216}
	\declarecolor{Orange}{237, 125, 49}
	\declarecolor{LightOrange}{251,229, 214}
	\declarecolor{Yellow}{255, 192, 0}
	\declarecolor{LightYellow}{255, 242, 200}
	\declarecolor{Blue}{91, 155, 213}
	\declarecolor{LightBlue}{222, 235, 247}
	\declarecolor{Green}{112, 173, 71}
	\declarecolor{LightGreen}{226, 240, 217}
	\declarecolor{Navy}{68, 114, 196}
	\declarecolor{LightNavy}{218, 227, 243}
	
	\newcommand{\declareperson}[1]{%
		\expandafter\newcommand\csname#1\endcsname[1]{\textcolor{Orange}{#1: ##1}}%
	}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikzsymbols}
	
	\usetikzlibrary{decorations}
	\usetikzlibrary{decorations.pathreplacing}
	\usetikzlibrary{decorations.markings}
	\usetikzlibrary{fit}
	\usetikzlibrary{intersections}
	\usetikzlibrary{matrix}
	\usetikzlibrary{overlay-beamer-styles}
	\usetikzlibrary{patterns}
	\usetikzlibrary{shapes}
	\usetikzlibrary{tikzmark}
	\usetikzlibrary{hobby}
	
	\usepgflibrary{arrows.meta}
	
	\tcbuselibrary{skins}
	\tcbuselibrary{raster}
	
	\usepgfplotslibrary{patchplots}
		
	\pgfdeclarelayer{background}
	\pgfdeclarelayer{foreground}
	\pgfsetlayers{background,main,foreground}
	\tikzstyle{na}=[baseline=-0.5ex]
	\tikzset{onslide/.code args={<#1>#2}{%
	  \only<#1>{\pgfkeysalso{#2}}
	}}
	\tikzset{temporal/.code args={<#1>#2#3#4}{%
	  \temporal<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}{\pgfkeysalso{#4}}
	}}
		
	\pgfplotsset{colormap={WhiteOrange}{
		color=(White)
		color=(Orange)
	}}
	\pgfplotsset{colormap={NavyOrange}{
		color=(LightNavy)
		color=(Orange)
	}}
	\pgfplotsset{colormap={WhiteNavy}{
		color=(White)
		color=(Navy)
	}}
	\pgfplotsset{colormap={WhiteBlack}{
		color=(White)
		color=(Black)
	}}
		
	\newcommand*{\Pic}[2][]{\begin{tikzpicture}\pic[#1]{#2};\end{tikzpicture}}
	\newcommand*{\sPic}[2]{\scalebox{#1}{\Pic{#2}}}
	\newcommand*{\cPic}[2][]{\begin{center}\Pic[#1]{#2}\end{center}}
	
	\newcommand{\rounded}[2][0.7ex]{%
		\begin{tikzpicture}
			\node[inner sep=0ex, draw=White, line width=0ex, opacity=0.] (a) {#2};
			\clip[rounded corners=#1] (a.south west) rectangle (a.north east);
			\node[inner sep=0ex] (a) {#2};
		\end{tikzpicture}%
	}
	
	\newcommand*{\tnode}[2]{\tikzmarknode{#1}{#2}}
}{}

\iftoggle{/opts/typesetting}{
	\iftoggle{presentation}{
	}{
		\RequirePackage{microtype}
		\RequirePackage[noblocks]{authblk}
		\RequirePackage{parskip}
		\RequirePackage{fullpage}
	}
	\RequirePackage{hyperref}
	\RequirePackage[capitalize, nameinlink]{cleveref}
	
	\iftoggle{/opts/colors}{
		\hypersetup{
			colorlinks=true,
			pdfpagemode=UseNone,
			citecolor=Green,
			linkcolor=Navy,
			urlcolor=Black
		}
	}{}
}{}

\iftoggle{/opts/theorems}{
	\iftoggle{presentation}{}{
		\theoremstyle{plain}
		\newtheorem{theorem}{Theorem}
		\newtheorem{lemma}[theorem]{Lemma}
		\newtheorem{corollary}[theorem]{Corollary}
		\newtheorem{proposition}[theorem]{Proposition}
		\newtheorem{fact}[theorem]{Fact}
		\newtheorem{conjecture}[theorem]{Conjecture}
		\newtheorem*{conjecture*}{Conjecture}
		
		\theoremstyle{definition}
		\newtheorem{definition}[theorem]{Definition}
		
		\theoremstyle{remark}
		\newtheorem{remark}[theorem]{Remark}
		\newtheorem{example}[theorem]{Example}
	}
}{}

\iftoggle{/opts/macros}{
	\providecommand{\given}{}
	\newcommand\GivenSymbol[1][]{%
		\nonscript\:#1\vert%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\providecommand{\mid}{}
	\newcommand\MidSymbol[1][]{%
		\nonscript\:#1\|%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\newcommand{\declaredelims}[3]{%
		\expandafter\DeclarePairedDelimiterX\csname#1\endcsname[1]{#2}{#3}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##1}%
	}
	
	\declaredelims{set}\{\}
	\declaredelims{card}\lvert\rvert
	\declaredelims{abs}\lvert\rvert
	\declaredelims{norm}\lVert\rVert
	\declaredelims{dotp}\langle\rangle
	\declaredelims{tuple}\lparen\rparen
	\declaredelims{parens}\lparen\rparen
	\declaredelims{bracks}\lbrack\rbrack
	
	\newcommand{\declarenameddelims}[4]{%
		\expandafter\DeclarePairedDelimiterXPP\csname#1\endcsname[1]{#2}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##1}%
		\expandafter\DeclarePairedDelimiterXPP\csname#1X\endcsname[2]{#2_{##1}}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##2}%
	}
	
	
	\let\Pr\relax
	\declarenameddelims{Pr}{\mathbb{P}}\lbrack\rbrack
	\declarenameddelims{Ex}{\mathbb{E}}\lbrack\rbrack
	
	\newcommand*{\eval}[1]{\left.#1\right\rvert}
	
	\iftoggle{presentation}{%
		\newcommand*{\mathdouble}[1]{\mathds{#1}}%
	}{%
		\newcommand*{\mathdouble}[1]{\mathbb{#1}}%
	}
	
	\let\Q\relax
	\newcommand*{\Q}{{\mathdouble{Q}}}
	\let\N\relax
	\newcommand*{\N}{{\mathdouble{N}}}
	\let\Z\relax
	\newcommand*{\Z}{{\mathdouble{Z}}}
	\let\R\relax
	\newcommand*{\R}{{\mathdouble{R}}}
	\let\C\relax
	\newcommand*{\C}{{\mathdouble{C}}}
	\let\1\relax
	\newcommand*{\1}{{\mathds{1}}}
	
	\let\poly\relax
	\DeclareMathOperator{\poly}{poly}
	\DeclareMathOperator{\supp}{supp}
	\DeclareMathOperator{\conv}{conv}
	\DeclareMathOperator{\rank}{rank}
	\let\Im\relax
	\DeclareMathOperator{\Im}{Im}
	\let\Re\relax
	\DeclareMathOperator{\Re}{Re}
}{}
\makeatother

